New spectral-parameter dependent solutions of the Yang-Baxter equation

The Yang-Baxter Equation (YBE) plays a crucial role for studying integrable many-body quantum systems. Many known YBE solutions provide various examples ranging from quantum spin chains to superconducting systems. Models of solvable statistical mechanics and their avatars are also based on YBE. Therefore, new solutions of the YBE could be used to construct new interesting 1D quantum or 2D classical systems with many other far-reaching applications. In this work, we attempt to find (almost) exhaustive set of solutions for the YBE in the lowest dimensions corresponding to a two-qubit case. We develop an algorithm, which can potentially be used for generating new higher-dimensional solutions of the YBE.

==> Sections/methodology-old.tex <==
The major idea behind our proposal is to identify the YBE solutions in such a manner that one avoids obtaining repeated solutions while having substantial control over the complexities of resolving an over-determined system of equations. 

We first recognized two different means of resolution: First to solve the relations as a set of differential equations and second to consider them as a system of polynomials that are reducible through Gr\"{o}bner basis calculations. Solving them exclusively by a single method is not feasible because of the excessive computational time that it takes. There is no systematic way to control the complexity of the obtained solutions, which further adds difficulties in their classification.

Hence, we choose a trade-off between these two methods by considering a branching algorithm that searches for \textit{solution vertices} in a graph of various \textit{search branches}. The algorithm starts with the initiation vertex having all the relations of Eq.~\eqref{eq:rels}. A subset of the relations are solved for developing various subcases. Each case represents a potential branch for further simplification which leads either to a solution of the YBE or an invalid end. The search branches are recursively generated until the algorithm exhausts all possibilities. An visualization of the branch search is provided in Fig.~\ref{fig:solbranch}. 

In this section, we provide the details of the involved workflow and showcase the main aspects of the algorithm. We have used the \verb|Mathematica| software to build the code base.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.25]{Figures/solbranches.png}
    \caption{A graph of search branches produced by the algorithm while searching for solutions of the YBE for an initial constraint (H14). The red dots indicate terminated vertices which may indicate a valid solution or an invalid (often indeterminate) one. The green dot is the \textit{initiation vertex} from where the algorithm initiated.}
    \label{fig:solbranch}
\end{figure}

\subsection{Computational Workflow}

\subsubsection*{Preparation}
The initial conditions $\mathcal{R}(0)$ chosen for resolving Eq.~\eqref{eq:rels} from Table~\ref{table:constantYBEsols} are assumed to be always invertible. It then enforces conditions on the parameters of the constant R-matrices. Then a complete set of relations is generated and separated in the following fashion - 

\begin{enumerate}
    \item Algebraic relations $\mathcal{A}(u)$ : $\mathcal{R}_{\textit{YBE}}(0,u), \mathcal{R}_{\textit{YBE}}(u,0)$
    \item Differential relations $\mathcal{D}(u)$ : $D[\mathcal{R}_{\textit{YBE}}(u,0),u], D[\mathcal{R}_{\textit{YBE}}(0,u),u], D[\mathcal{R}_{\textit{YBE}}(u,v),v]_{v\rightarrow 0},\\ D[\mathcal{R}_{\textit{YBE}}(v,u),v]_{v\rightarrow 0}$
    \item Initial condition of differential relations $\mathcal{D}(0)$
\end{enumerate}
Any relations in $\mathcal{D}(u)$ and $\mathcal{D}(0)$, which has no differential form is shifted in $\mathcal{A}(u)$.

\subsubsection*{Initialisation}
The initialization vertex is generated with all considered relations. The algorithm then decides to evaluate a subset of relations from the algebraic relations $\mathcal{A}(u)$ in accordance below
\begin{itemize}
      \item If the relations in $\mathcal{A}(u)$ is less than a specified range $N_{\text{lim}}$, then we choose to compute their Gr\"{o}bner basis first.
      \item If it is not the case, then a subset of relations having a linear or factorised form is considered. It is under a limit of its \textit{complexity length} which is determined by the number of the terms involved. The maximal length is denoted by $N_{\text{term}}$.
\end{itemize}
The chosen set is further solved by employing \verb|Reduce[]| method in the Mathematica. The results then go through a series of evaluations for checking if they solve the complete relation set. Those which do so are labelled as solutions of Eq.~\eqref{eq:RRRdiff}. Results with indeterminate terms or invalid logic are terminated. The rest of the search branches are considered for the next iteration. To solve the issue of repeated solutions, any branches having the identical contents in their relation set are merged.

\subsubsection*{Iteration}

The collection of unresolved branches go through a similar process of simplification as described in the former section. However there are central differences from the initialisation stage. For every branch, their relation set are separated as $\mathcal{D}(u), \mathcal{D}(0)$ and $\mathcal{A}(u)$, exactly like in the preparation stage. To simplify every branch for further subcases, the algorithm considers the following scheme:
\begin{itemize}
    \item A subset of relations from $\mathcal{A}(u)$ having a linear or factorised form and satisfying their complexity length lesser than $N_{\text{term}}$ is evaluated first. 
    \item If no such relations are available then the algorithm tries computing Gr\"{o}bner basis for the relations in $\mathcal{A}(u)$ if it is lesser than or equal to $N_{\text{lim}}$.
    \item If the relations in $\mathcal{A}(u)$ is larger than $N_{\text{lim}}$, then the algorithm uses \verb|DSolve[]| method from Mathematica to solve relations from $\mathcal{D}(u)$ and $\mathcal{D}(0)$ whose complexity length is lesser than $N_{\text{diff}}$
    \item Otherwise it terminates solving for this branch and proceeds for the next unresolved case.
\end{itemize}
The algorithm goes through the same process of evaluation for filtering resolved solutions, terminating indeterminate or invalid cases, building new search branches and merging identical results. The algorithm reiterates to generate new extensions and continues until there are no new unresolved branches. The final outcome of the computation are stored in an accessible \verb|Association[]| graph object in Mathematica which contains all details of the evaluation. The algorithm gathers all solution vertices in every iterative run. We summarise the algorithm's workflow in Fig.~\ref{fig:RRRworkflow}.

\subsubsection*{Finalisation}
The algorithm is executed for every initial condition as from Table~\ref{table:constantYBEsols}. All valid YBE solutions from each condition are collated. By using the symmetries of the R-matrices, redundant cases are removed. Finally, we obtain a list of unique R-matrices. 

\tikzstyle{initialise} = [rectangle, rounded corners, minimum width=4cm, minimum height=1cm,text centered, draw=black, fill=yellow!30]
\tikzstyle{process} = [rectangle, rounded corners, minimum width=4cm, minimum height=1cm, text centered, text width=5cm, text width=3cm, draw=black, fill=orange!30]
\tikzstyle{stopped} = [rectangle, rounded corners,  minimum width=4cm, minimum height=1cm, text centered, draw=black, fill=red!30]
\tikzstyle{decision} = [diamond, minimum width=1cm, minimum height=1cm, text centered, text width=2cm, draw=black, fill=yellow!30]
\tikzstyle{arrow} = [thick,->,>=stealth]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tikzpicture}[node distance=1.8cm,auto]
\node (init) [initialise] {Initialise conditions};
\node (rels) [process, below of=init] {Frame initial relations};
\node (meth) [process,below of=rels] {Choosing Method of Evaluation};
\node (redc) [process,below of=meth] {Reduction of equations};
\node (fitr) [process,below of=redc] {Filtering Ansatzes};
\node (branch) [process,below of=fitr] {Branching solutions};
\node (node) [decision,below of=branch, yshift=-1cm] {Unresolved branches?};
\node (end) [stopped,below of=node,yshift=-1cm] {End};

\draw [arrow] (init) -- (rels);
\draw [arrow] (rels) -- (meth);
\draw [arrow] (meth) -- (redc);
\draw [arrow] (redc) -- (fitr);
\draw [arrow] (fitr) -- (branch);
\draw [arrow] (branch) -- (node);
\draw [arrow] (node) -- node[anchor=east] {No} (end);
\draw [arrow] (node) -- +(+2.3,0) |- node[anchor=west] {Yes} (meth);
\end{tikzpicture}
\captionof{figure}{Summary of the workflow of the algorithm}
\label{fig:RRRworkflow}
\end{center}
\end{minipage}

\subsection{Algorithm's determinants and its limitations}
We summarise all the constraints that are involved in the execution of the algorithm with their default parameters used 
\begin{enumerate}
    \item The complexity length of a algebraic relation, $N_{\text{term}}$ (4)
    \item The complexity length of a differential relation, $N_{\text{diff}}$ (8)
    \item The number of relations for Gr\"{o}bner basis computations, $N_{\text{lim}}$ (24)
    \item Time limit for running Gr\"{o}bner basis computations, $t_{\text{gb}}$ (20 mins)
    \item Time limit for running \verb|Reduce[]| method, $t_{\text{rd}}$ (5 min)
\end{enumerate}
Alongside with the initial condition $\mathcal{R}(0)$, we have the complete set of determinants of the algorithm. One may adjust these parameters for an extensive algorithmic search, which further depends on the available hardware configurations on which the programs are executed. 

\subsubsection*{Advantages}

We then infer the limitations of the algorithm from these determinants. Using $N_{\text{term}}$ and $N_{\text{diff}}$ in a larger setting will not influence the algorithm significantly, as it leads to lesser iterative steps for algebraic simplification at the cost of increasing the number of search branches per execution.

The important constraints are $N_{\text{lim}}$ and both time limits. Since they cap the scope of solving difficult time-consuming relations, the algorithm may not be able to finish resolving certain terminated branches. An notable feature of this process is that all terminated search branches from the final output of the program can be re-executed with broader determinants. Hence one can extend the incomplete tedious algorithmic search in the future.

\subsubsection*{Shortcomings and Scopes}
The shortcomings comes mainly from developing custom pattern-based filters to identify complicated set of relations which are either used to avoid untenable search branches or to simplify them further. These methods are additionally developed which then provides future scopes for customising the algorithm. 

In the context of this work, we have avoided dealing with nonlinear relations (those with power terms) explicitly and considered simplifying them through Gr\"{o}bner computations. Square-root sub-expressions are tended by assuming them to be positive, as every branch cut of such terms are already considered in the \verb|Reduce[]| method. 

In this manner, the algorithm only dealt with linearised relations from where the R-matrices are computed. Hence we could present a \textit{sufficiently exhaustive} search for all spectral solutions of the YBE.

We also considered cases where the spectral R-matrices are invertible. The main reason is that the we assumed that the initial condition $\mathcal{R}(0)$ of these solutions are invertible. In general, one may relax this requirement. Hence there are future scopes in finding new results with new non-invertible initial conditions. 


==> Sections/solution-method.tex <==
\subsection{Main solution stages}

Main solution stages are the following (see Algorithm~\ref{alg:mainstages}).
\begin{enumerate}
	\item  Select constant solution as initial conditions.
	\item  Solve the initial YBEs (\ref{eq:dRRR1})--(\ref{eq:dRRR4}). 
		\label{alg:stage2}
	\item Solve the one-variable algebraic and the differential YBEs (\ref{eq:algRRR1})--(\ref{eq:algRRR2}) step-by-step.
		\label{alg:stage3}
	\item Substitute obtained solutions to (\ref{eq:RRRdiff}) and solve the residual equations if it exists.
\end{enumerate}
Both Stages~\ref{alg:stage2} and \ref{alg:stage3} have much in common. Later we describe Stage~\ref{alg:stage3} and present the corresponding diagram. Description of Stage~\ref{alg:stage2} is given in Appendix.

\begin{algorithm}
	\caption{Main solution stages \label{alg:mainstages}}
	\begin{algorithmic}[1]
		\State Select constant solution as initial conditions
		\State Solve the initial YBEs (\ref{eq:dRRR1})--(\ref{eq:dRRR4}) 
		\State Solve the one-variable algebraic and the differential YBEs (\ref{eq:algRRR1})--(\ref{eq:algRRR2}) step-by-step 
		\State Substitute obtained solutions to (\ref{eq:RRRdiff}) and solve the residual equations if it exists.
	\end{algorithmic}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[hbt]
% %\begin{minipage}{0.5\textwidth}
% \begin{center}
% \begin{tikzpicture}[node distance=2cm,auto]
% 	\node (init) [initialise] {Start};
% 	\node (initConditions) [process, below of=init] {Select constant solution as initial conditions};
% 	\node (initYBEs) [process,below of=initConditions] {Solve the initial YBEs (\ref{eq:dRRR1})--(\ref{eq:dRRR4}) };
% 	\node (mainSolution) [process,below of=initYBEs] {Solve the one-variable algebraic and the differential 
% 		YBEs (\ref{eq:algRRR1})--(\ref{eq:algRRR2}) step-by-step};
% 	\node (checks) [process,below of=mainSolution] {Substitute obtained solutions to (\ref{eq:RRRdiff}) and 
% 		solve the residual equations, if it exists};
% 	\node (end) [stopped,below of=checks] {End};
% 	%	
% 	\draw [arrow] (init) -- (initConditions);
% 	\draw [arrow] (initConditions) -- (initYBEs);
% 	\draw [arrow] (initYBEs) -- (mainSolution);
% 	\draw [arrow] (mainSolution) -- (checks);
% 	\draw [arrow] (checks) -- (end);
% \end{tikzpicture}
% \captionof{figure}{General workflow }
% \label{fig:GWorkflow}
% \end{center}
% %\end{minipage}
% %\hfill\,\hfill
% \end{figure}


\subsection{Methodology of solving one-variable algebraic and the differential YBEs}

The major idea behind our proposal is to identify the YBE solutions in such a manner that one avoids obtaining repeated solutions while having substantial control over the complexities of resolving an over-determined system of equations. 

We first recognize two different means of resolution: First to solve the relations as a set of differential equations and secondly to consider them as a system of polynomials that are reducible through Gr\"obner basis calculations. Solving them exclusively by a single method is not feasible because of the excessive computational time that it takes. There is no systematic way to control the complexity of the obtained solutions, which further adds difficulties in their classification.

Hence, we choose a trade-off between these two methods by considering a branching algorithm, which searches for \textit{solution vertices} in a graph of various \textit{search branches}. The algorithm starts with the initiation vertex having all the relations of Eq.~\eqref{eq:rels}. A subset of the relations is solved for developing various subcases. Each case represents a potential branch for further simplification which leads either to a solution of the YBE or an invalid end. The search branches are recursively generated until the algorithm exhausts all possibilities. A visualization of the branch search is provided in Fig.~\ref{fig:solbranch}. 

In this section, we provide the details of the involved workflow and showcase the main aspects of the algorithm. We have used the \verb|Mathematica| software to build the code base.

\subsection{Algorithm and workflow of solving one-variable algebraic and the differential YBEs}

\subsubsection{Main idea}

The idea is to solve equations step-by-step. For every step, choose `a few' `simple' equations from a set of differential and algebraic equations and solve them. Obtained solution substitute to a set of differential and algebraic equations. The notion of `a few` as well as `simple' is to be clarified later. The id of the step is its number. We can have more than one solution for every step, so we have a branching solution presented by some graphs.

\subsubsection{Data structures}
$\Ids{dRRRList}[i]$ --- a list of differential  YBEs at step $i$.\\
$\Ids{algRRRList}[i]$ --- a list of one-variable algebraic YBEs at step $i$.\\
%$\mathtt{initDRRRList[i]}$ --- a list of initial YBEs at step $i$.
$\Ids{RmGraph}$ --- a graph of solution process. Every vertex of the graph $\Ids{RmGraph}$ has boolean properties 
$\Idc{Stopped}$, $\Idc{TempStopped}$ and $\Idc{Finalized}$ or not, that means we have a contradiction or (partially) final solution correspondingly.\\
Temporal variables:\\
$\Ids{tmpEqnsList}[i]$ --- a list of equations to be solved for vertex $i$.\\
$\Ids{doVertList}$ ---  a list of vertices of the graph $\mathtt{RmGraph}$ to be considered during the current cycle (see below ...).\\
$\mathtt{tmpEqnsList}[i]$ --- a list of equations to be solved for vertex $i$.\\
$\textnormal{\ttfamily tmpEqnsList}[i]$ --- a list of equations to be solved for vertex $i$.\\
$\Id{doVertList}$ ---  a list of vertices of the graph $\Id{RmGraph}$ to be considered during the current cycle (see below ...).\\
\Id{method} --- global variable.

\subsubsection{Algorithm and workflow of stage \ref{alg:stage3}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
	\caption{Stage 3 \label{alg:stage3}}
	\begin{algorithmic}[1]
		\Description Algorithm of Stage 3
		\Input %
		\Output %
		\Require %something
		\Ensure %something
		\Statex
		\Statex Local \Ids{doNewVertList}
		\Comment{To store new vertices}
		\State $\Ids{doVertList} \gets 
			\Call{GetToDoVertices}{\Ids{RmGarph}}$ 
		%\Statex \Comment{(Is any non-$\Idc{Stopped}$, non-$\Idc{TempStopped}$ and not-$\Idc{Finalized}$  
		%	vertex without child vertices?)}
		\While{$\Ids{doVertList}$ is not empty }
			\Statep{$\Id{method} \gets$ 
				\Call{SelectEqnsToSolve}{\Ids{dRRRList},  \Ids{algRRRList}, \Ids{tmpEqnsList}, \Ids{doVertList}} 
			\Comment{Select method to solve, select equations to solve}}
			\State \Call{ReduceVertexEqns}{\Ids{tmpEqnsList}, \Ids{doVertList}, \Ids{rSolution}}
			\State \Call{ProcSolutions}{\Ids{RmGarph}, \Ids{rSolution}, \Ids{algRRRList}, \Ids{dRRRList}, \Ids{doVertLst}}
			\State $\Ids{doNewVertList} \gets \Call{GetNewVertices}{\Ids{RmGarph}, \Ids{doVertList}}$
			\State \Call{UniteVertices}{\Ids{RmGarph}, \Ids{doNewVertList}}
			\State $\Ids{doNewVertList} \gets \Call{GetNewVertices}{\Ids{RmGarph}, \Ids{doVertList}}$
			\State \Call{TransformEquationsLists}{\Ids{algRRRList}, \Ids{dRRRList}, \Ids{doNewVertList}}
			\State $\Ids{doVertList} \gets  \Call{GetToDoVertices}{\Ids{RmGarph}}$
		\EndWhile
		\ForAll{$i \in \Ids{RmGraph}$ and marked as \Idc{TempStopped}}
			\State Unmark vertex $i$ as \Idc{TempStopped}
		\EndFor
	\end{algorithmic}
\end{algorithm}



%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[hbtp]
%\begin{minipage}{0.5\textwidth}
\begin{center}
\small
\tikzstyle{process} = [rectangle, rounded corners, minimum width=4cm, minimum height=1cm,
	 text centered, text width=0.3\linewidth, draw=black, fill=yellow!20]
\tikzstyle{coord}=[coordinate]%{coordinate, on chain, on grid, node distance=6mm and 25mm}
\begin{tikzpicture}[node distance=1.75cm,auto]
	\node (init) [initialise] {Start};
	\node (doVertList1)[process, below of=init, text width=0.5\linewidth]{$\Ids{doVertList}\leftarrow$ list of   
		non-$\Idc{Stopped}$, non-$\Idc{TempStopped}$ and not-$\Idc{Finalized}$  vertices};
	\node(isEmpty)[decision, below of=doVertList1,yshift=-1.3cm]{Is $\Ids{doVertList}$ empty?};
	\node(methodSelection)[process, below of=isEmpty, yshift=-1.5cm, text width=0.3\linewidth]{
		Select equations to solve and corresponding method};
	\node(GBmethod)[decision,below of=methodSelection, yshift=-1.5cm]{\Id{method} = ``Gr\"obner basis''?};
	\node(computeGBasis)[process, right of=GBmethod, text width=0.3\linewidth, xshift=4cm]{Compute Gr\"obner basis 
		for selected equations};
	\node(afterGBmethod)[coord, below of=GBmethod, yshift=-0.5cm]{};
	\node(Dmethod)[decision,below of=afterGBmethod, yshift=-0.5cm]{\Id{method} = ``Differential equation''?};
	\node(SolveHD)[process, right of=Dmethod, text width=0.3\linewidth, xshift=4.5cm]{Solve with respect to 
		higher derivatives};
	\node(algSolve)[process, below of=Dmethod, yshift=-1.5cm, text width=0.3\linewidth]{Solve algebraic equations};
	\node(DSolve)[process, right of=algSolve, text width=0.3\linewidth, xshift=4.5cm]{Solve differential equation};
	\node(afterAlgSolve)[coordinate, below of=algSolve, node distance=1.2cm]{};
	\node(addNewVertices)[process, below of=afterAlgSolve, node distance=1.2cm, text width=0.6\linewidth]{Add 
		new vertices, check solutions,  unite vertices, transform equations};
	\node(unmark)[process, right of=isEmpty, xshift=4cm, text width=0.3\linewidth]{Unmark all vertices 
		marked as \Idc{TempStopped}};
	\node(end)[stopped, below of=unmark]{End};
	%
	\draw [arrow] (init) -- (doVertList1);
	\draw [arrow] (doVertList1) -- (isEmpty);
	\draw [arrow] (isEmpty) -- node(isEmptyNo)[anchor=east]{No} (methodSelection);
	\draw [arrow] (methodSelection) -- (GBmethod);
	\draw [arrow] (GBmethod.east) -- node{Yes} (computeGBasis.west);
	\draw [arrow,-] (GBmethod) -- node[anchor=east]{No}(afterGBmethod);
	\draw [arrow,->o] (computeGBasis) |- (afterGBmethod.west);
	\draw [arrow] (afterGBmethod) -- (Dmethod);
	\draw [arrow] (Dmethod) -- node{yes} (SolveHD.west);
	\draw [arrow] (SolveHD) -- (DSolve);
	\draw [arrow] (Dmethod) -- node[anchor=east]{No} (algSolve);
	\draw [arrow,-] (algSolve) -- (afterAlgSolve);
	\draw [arrow,->o] (DSolve) |- (afterAlgSolve.east);
	\draw [arrow] (afterAlgSolve) -- (addNewVertices);
	\draw [arrow] (addNewVertices) -- +(-6,0) |- (doVertList1);
	\draw [arrow] (isEmpty.east) -- node(isEmptyYes){Yes} (unmark);
	\draw[arrow] (unmark) -- (end);
\end{tikzpicture}
\captionof{figure}{Stage 2 workflow}
\label{fig:Stage2Workflow}
\end{center}
%\end{minipage}
%\hfill
%\,\hfill
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
	\caption{Code of GetToDoVertices function}
	\begin{algorithmic}[1]
		\Description %Evaluates and prints the factorial of $n$ 
		\Input $\Ids{RmGarph}$ %A non-negative integer number $n$
		\Output list of vertices to be processed %The value of the factorial $n$
		\Require $\Ids{RmGarph}$ exists%something
		\Ensure %something
		\Statex
		\Function{GetToDoVertices}{$\Ids{RmGarph}$}
			\State Local $\Ids{tmpList}\gets$  empty list 
			%\State ${tmpList}\gets$  empty list 
			%\State $\textit{tmpList}\gets$  empty list 
			%\State $\mathtt{tmpList}\gets$  empty list 
			%\State $\textnormal{\ttfamily tmpList}\gets$  empty list 
			\ForEach{$i \in$ vertices of  $\Ids{RmGraph}$}
				\If{(vertex $i$  has not child vertices) \textbf{and} (vertex $i$ is not marked as \Idc{Stopped} 
						or \Idc{TempStopped} or \Idc{Finalized})}
					%\State Append $i$ to  $\Ids{tmpList}$
					\State $\Ids{tmpList} \gets \Ids{tmpList} \cup i$
					\Comment{Append $i$ to  $\Ids{tmpList}$}
				\EndIf
			\EndFor
			\State \Return $\Ids{tmpList}$
		\EndFunction
	\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
	\caption{Selection of equations to solve and method for solving \label{alg:methodSelect}}
	\begin{algorithmic}[1]
	\small
		\Description Select equations to solve and corresponding method
		\Input \Ids{dRRRList}, \Ids{algRRRList}, \Ids{doVertList}
		\Output updates \Ids{tmpEqnsList} and set global variable \Id{method}
		\Require $\forall i \in \Ids{doVertLst}: (\Call{Length}{\Ids{algRRRList}[i]} > 0$) 
			\textbf{or} ($\Call{Length}{\Ids{dRRRList}[i]} > 0$)
		\Ensure %something
		\Statex 
		\Procedure{SelectEqnsMethodToSolve}{$\Ids{dRRRList}$, $\Ids{algRRRList}$, 
				$\Ids{tmpEqnsList}$, \Ids{doVertList}}
			\State Local \Ids{eqnsCountList}
			\Comment{contains number of selected equations}
			\State $\Ids{eqnsCountList} \gets \text{empty list}$
			\ForEach{$i \in \Ids{doVertList}$}
				\Statep{$\Ids{tmpEqnsList}[i] \gets$ linear in $\mathcal{R}_{j_{1} j_{2}}^{k_{1} k_{2}}(u) $ 
					equations from $\Ids{algRRRList}[i]$ having no more than $N_{\mathrm{term}}$ terms 
					in expanded form}
				\State $\Ids{eqnsCountList} \gets \Ids{eqnsCountList} \cup  \Call{Length}{\Ids{tmpEqnsList}[i]}$
				\Statex \Comment{append \Call{Length}{\Ids{tmpEqnsList}[i]} to \Ids{eqnsCountList}}
			\EndFor
			\If{\Ids{eqnsCountList} has non-zero elements}
				\State $\Id{method} \gets \TextString{Linear method}$
				\Comment{Linear method}
			\Else
				\ForEach{$i \in \Ids{doVertList}$}
					\Statep{$\Ids{tmpEqnsList}[i] \gets$ factorizable equations from $\Ids{algRRRList}[i]$}
					\State $\Ids{eqnsCountList} \gets \Ids{eqnsCountList} \cup  \Call{Length}{\Ids{tmpEqnsList}[i]}$
					%\Statex \Comment{append \Call{Length}{\Ids{tmpEqnsList}[i]} to \Ids{eqnsCountList}}
				\EndFor
				\If{\Ids{eqnsCountList} has non-zero elements}
					\State $\Id{method} \gets \TextString{Product method}$
					\Comment{Product method}
				\Else
					\ForEach{$i \in \Ids{doVertList}$}
						\If{$\Call{Length}{\Ids{algRRRList}[i]}<N_{\mathrm{lim}}$	}
							\State $\Ids{tmpEqnsList}[i] \gets \Ids{algRRRList}[i]$
							\Comment{$N_{\mathrm{lim}}$ is a tuning parameter}
						\Else
							\State $\Ids{tmpEqnsList}[i] \gets \text{empty list}$	
						\EndIf
						\State $\Ids{eqnsCountList} \gets \Ids{eqnsCountList} \cup  
							\Call{Length}{\Ids{tmpEqnsList}[i]}$
						%\Statex \Comment{append \Call{Length}{\Ids{tmpEqnsList}[i]} to \Ids{eqnsCountList}}
					\EndFor
					\If{\Ids{eqnsCountList} has non-zero elements}
						\State $\Id{method} \gets \TextString{Gr\"obner basis method}$
						\Comment{Gr\"obner basis method}
					\Else
						\ForEach{$i \in \Ids{doVertList}$}
							\Statep{$\Ids{tmpEqnsList}[i] \gets$ one shortest equation from $\Ids{dRRRList}[i]$
								and having no more than $N_{\mathrm{diff}}$ terms in expanded form}
							\State $\Ids{eqnsCountList} \gets \Ids{eqnsCountList} \cup  1$
							\Comment{append $1$ to \Ids{eqnsCountList}}
							%\Statex \Comment{append $1$ to \Ids{eqnsCountList}}
						\EndFor
						\If{\Ids{eqnsCountList} has non-zero elements}
							%\Statex \Comment{Differential equation method}
							\Statep[Differential equation method]{$\Id{method} \gets 
								\TextString{Differential equation method}$}
						\Else
							\State Break algorithm
						\EndIf
					\EndIf
				\EndIf
			\EndIf
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
	\caption{ReduceVertexEqns}
	\begin{algorithmic}[1]
		\Description Solve selected equations
		\Input \Ids{tmpEqnsList}, \Ids{dovertList}
		\Output append obtained solutions to \Ids{rSolution}
		\Require $\Ids{tmpEqnsList}[i]$ is not empty $\forall i \in \Ids{doVertList}$
		\Ensure %something
		\Statex 
		\Procedure{ReduceVertexEqns}{\Ids{tmpEqnsList}, \Ids{doVertList}, \Ids{rSolution}}
			\State Local \Id{tmpDEqn}, \Ids{tmpDEqns}
			\Statex \Comment{\parbox[t]{\dimexpr\longcommentlength}{To store current differential equation 
					to be algebraically solved  	with  respect to higher derivatives and all differential equations}}
			\ForEach{$i \in \Ids{doVertList}$}
				\If{$\Id{method}\neq \TextString{Differential equation method}$}
					\State $\Ids{rSolution}[i]\gets \Call{Solve}{\Ids{tmpEqnsList}[i]}$
					\Comment{Solve algebraic equations}
				\Else
					\State $\Ids{tmpDEqns}\gets \Call{Solve}{\Ids{tmpEqnsList}[i]}$
					\Statex \Comment{Algebraically solve differential equation with respect to higher derivatives}
					\ForEach{\Id{tmpDEqn} in \Ids{tmpDEqns}}
						\State $\Ids{rSolution}[i]\gets  \Ids{rSolution}[i] \cup \Call{DiffSolve}{\Id{tmpDEqn}}$
						\Statex \Comment{Solve differential equation and append obtained solution 
							to $\Ids{rSolution}[i]$}
					\EndFor
				\EndIf
				\If{$\Ids{rSolution}[i]$ is empty list}
					\State Mark vertex $i$ as \Idc{Stopped}
					\Comment{No solutions}
				\EndIf
			\EndFor
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
	\caption{Process obtained solutions}
	\begin{algorithmic}[1]
		\Description Add vertices to the graph. One vertex for every new solution.
		\Input \Ids{RmGarph}, \Ids{rSolution}, \Ids{algRRRList}, \Ids{dRRRList}, \Ids{doVertLst} 
		\Output Updates \Ids{algRRRList}, \Ids{dRRRList}
		\Require $\Ids{RmGarph}$ exists%something
		\Ensure %something
		\Statex
		\Procedure{ProcSolutions}{\Ids{RmGarph}, \Ids{rSolution}, \Ids{algRRRList}, \Ids{dRRRList}, \Ids{doVertLst}}
			\State Local \Id{tmpSol}
			\Comment{Local variable to store current solution}
			%\Statep[Local variable for  solution number]{Local $j$}
			\State $j\gets$ number of vertices of \Ids{RmGraph}
			\ForEach{$i \in \Ids{doVertList}$}
				%\State $N\gets$ number of vertices of \Ids{RmGraph}
				%\State $j\gets 1$
				\ForEach{$\Ids{tmpSol} \in \Ids{rSolution}[i]$}
					\State $j \gets j + 1$
					\Statep{Append new vertex $j$ to graph \Ids{RmGraph} }
					\Statep{Add directed edge from vertex $i$ to child vertex $j$}
					\Statep{$\Ids{algRRRList}[j] \gets$ substitute \Ids{tmpSol} to $\Ids{algRRRList}[i]$}
					\Statep{$\Ids{dRRRList}[j] \gets$ substitute \Ids{tmpSol} to $\Ids{dRRRList}[i]$}
					\If{(obtained solution leads to degenerate or singular $\mathcal{R}$-matrix) \textbf{or} 
						($\Ids{algRRRList}[i]$ is singular) \textbf{or} 
						($\Ids{algRRRList}[i]$ is singular)
						}
						\Statep{Mark vertex $j$ as \Idc{Stopped}}
					\EndIf
				\EndFor
			\EndFor
			%\State \Return $\Ids{tmpList}$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
	\caption{Code of GetNewVertices function}
	\begin{algorithmic}[1]
		\Description %Evaluates and prints the factorial of $n$ 
		\Input \Ids{RmGraph}, \Ids{doVertList} %A non-negative integer number $n$
		\Output list of new vertices  %The value of the factorial $n$
		\Require \Ids{RmGarph} exists \textbf{and} \Ids{doVertList} is not empty%something%something
		\Ensure %something
		\Statex
		\Function{GetNewVertices}{\Ids{RmGarph}, \Ids{doVertList}}
			\State Local $\Ids{tmpList}\gets$  empty list 
			\ForEach{$i \in$ \Ids{doVertList}}
				\ForAll{$j \in$ child vertices of vertex $i$ of \Ids{RmGraph}}
					\If{(vertex $i$  has not child vertices) \textbf{and} (vertex $i$ is not marked as \Idc{Stopped} 
						or \Idc{TempStopped} or \Idc{Finalized})}
						\State $\Ids{tmpList} \gets \Ids{tmpList} \cup i$
						\Comment{Append $i$ to  $\Ids{tmpList}$}
					\EndIf
				\EndFor
			\EndFor
			\State \Return $\Ids{tmpList}$
		\EndFunction
	\end{algorithmic}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
	\caption{Code of UniteVertices}
	\begin{algorithmic}[1]
		\Description %Evaluates and prints the factorial of $n$ 
		\Input \Ids{RmGraph}, \Ids{doNewVertList} %A non-negative integer number $n$
		\Output Updates \Ids{RmGraph}
		\Require %\Ids{RmGarph} exists \textbf{and} \Ids{doVertList} is not empty%something%something
		\Ensure %something
		\Statex
		\Procedure{UniteVertices}{\Ids{RmGarph}, \Ids{doNewVertList}}
			\State Local $\Ids{tmpList}\gets$  empty list 
			\ForEach{$i \in \Ids{RmGraph}$}
				\ForAll{$j \in \Ids{doVertList}$, $j>i$}
					\If{($j \not\in \Ids{tmpList}$) \textbf{and} (edge between vertices $j$ and $i$ does not exist)}
						%\textbf{and} (vertices $i$ and $j$ leads to the same $\mathcal{R}$-matrix)}
						\If{vertices $i$ and $j$ leads to the same $\mathcal{R}$-matrix}
							\State $\Ids{tmpList}\gets \Ids{tmpList} \cup j$
							\Comment{Append $j$ to \Ids{tmpList}}
							\State Add directed edge from vertex $j$ to vertex $i$ in \Ids{RmGraph}
						\EndIf
					\EndIf
				\EndFor
			\EndFor
			%\State %\Return $\Ids{tmpList}$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
	\caption{Code of TransformEquationsLists}
	\begin{algorithmic}[1]
		\Description %Evaluates and prints the factorial of $n$ 
		\Input \Ids{algRRRList}, \Ids{dRRRList}, \Ids{doNewVertList} 
		\Output Updates \Ids{algRRRList}, \Ids{dRRRList}
		\Require %\Ids{RmGarph} exists \textbf{and} \Ids{doVertList} is not empty%something%something
		\Ensure %something
		\Statex
		\Procedure{TransformEquationsLists}{\Ids{algRRRList}, \Ids{dRRRList}, \Ids{doNewVertList}}
			%\State Local $\Ids{tmpList}\gets$  empty list 
			\ForEach{$i \in \Ids{doNewVertList}$}
				\State Remove constant non-zero factors for every expression in $\Ids{algRRRList}[i]$
				\State Remove zeros from $\Ids{algRRRList}[i]$
				\State Remove constant non-zero factors for every expression in $\Ids{dRRRList}[i]$
				\State Remove zeros from $\Ids{algRRRList}[i]$
				\If{some expression in $\Ids{algRRRList}[i]$ or in $\Ids{dRRRList}[i]$ is non-zero constant}
					\State Mark vertex $i$ as \Idc{Stopped}
				\EndIf
				\If{both \Ids{algRRRList} and \Ids{dRRRList} are empty lists}
					\State Mark vertex $i$ as \Idc{TempStopped}
				\EndIf
			\EndFor
			%\State %\Return $\Ids{tmpList}$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\clearpage



